Tips and Tricks for Visual Question Answering: Learnings from the 2017 Challenge

This paper presents a state-of-the-art model for visual question answering (VQA), which won the first place in the 2017 VQA Challenge. VQA is a task of significant importance for research in artificial intelligence, given its multimodal nature, clear evaluation protocol, and potential real-world applications. The performance of deep neural networks for VQA is very dependent on choices of architectures and hyperparameters. To help further research in the area, we describe in detail our high-performing, though relatively simple model. Through a massive exploration of architectures and hyperparameters representing more than 3,000 GPU-hours, we identified tips and tricks that lead to its success, namely: sigmoid outputs, soft training targets, image features from bottom-up attention, gated tanh activations, output embeddings initialized using GloVe and Google Images, large mini-batches, and smart shuffling of training data. We provide a detailed analysis of their impact on performance to assist others in making an appropriate selection.

==> modell-vqa4-100-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-reference-ensbl1.tex <==
63.21 $\pm$0.00   &  80.29  &  42.82  &  55.77  &  34.79 

==> modell-vqa4-100-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-reference-ensbl2.tex <==
63.19 $\pm$0.00   &  80.08  &  42.98  &  55.83  &  34.58 

==> modell-vqa4-100-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-reference-ensbl3.tex <==
63.06 $\pm$0.00   &  79.82  &  42.81  &  55.83  &  34.59 

==> modell-vqa4-105-b1s1o8vg0-g300e512-e-1_60_1_51_1_-8-a1-noVg-ensbl1.tex <==
62.56 $\pm$0.00   &  80.75  &  41.89  &  54.36  &  34.46 

==> modell-vqa4-105-b1s1o8vg0-g300e512-e-1_60_1_51_1_-8-a1-noVg-ensbl2.tex <==
62.57 $\pm$0.00   &  80.35  &  42.21  &  54.60  &  34.20 

==> modell-vqa4-105-b1s1o8vg0-g300e512-e-1_60_1_51_1_-8-a1-noVg-ensbl3.tex <==
62.31 $\pm$0.00   &  80.02  &  42.08  &  54.35  &  33.70 

==> modell-vqa4-110-b0s0o8vg1-g300e512-e-1_60_1_51_1_-8-a1-balancedShuffling0-ensbl1.tex <==
63.28 $\pm$0.00   &  80.29  &  43.07  &  55.84  &  34.73 

==> modell-vqa4-110-b0s0o8vg1-g300e512-e-1_60_1_51_1_-8-a1-balancedShuffling0-ensbl2.tex <==
63.21 $\pm$0.00   &  80.36  &  42.66  &  55.76  &  34.86 

==> modell-vqa4-110-b0s0o8vg1-g300e512-e-1_60_1_51_1_-8-a1-balancedShuffling0-ensbl3.tex <==
63.36 $\pm$0.00   &  80.33  &  43.06  &  55.98  &  34.94 

==> modell-vqa4-110-b0s0o8vg1-g300e512-e-1_60_1_51_1_-8-a1-balancedShuffling0.tex <==
63.28 $\pm$0.07   &  80.33  &  42.93  &  55.86  &  34.84 

==> modell-vqa4-115-b-1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-balancedShuffling-1-ensbl1.tex <==
63.10 $\pm$0.00   &  80.16  &  42.42  &  55.76  &  34.46 

==> modell-vqa4-115-b-1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-balancedShuffling-1-ensbl2.tex <==
63.22 $\pm$0.00   &  80.25  &  43.47  &  55.64  &  34.62 

==> modell-vqa4-115-b-1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-balancedShuffling-1-ensbl3.tex <==
63.15 $\pm$0.00   &  80.10  &  42.87  &  55.79  &  34.53 

==> modell-vqa4-120-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-minAcc.1-ensbl1.tex <==
63.23 $\pm$0.00   &  80.17  &  42.81  &  55.90  &  34.79 

==> modell-vqa4-120-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-minAcc.1-ensbl2.tex <==
63.18 $\pm$0.00   &  80.27  &  42.70  &  55.75  &  34.78 

==> modell-vqa4-120-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-minAcc.1-ensbl3.tex <==
63.24 $\pm$0.00   &  80.21  &  43.11  &  55.81  &  34.77 

==> modell-vqa4-120-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-minAcc.1.tex <==
63.22 $\pm$0.03   &  80.22  &  42.87  &  55.82  &  34.78 

==> modell-vqa4-125-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-minAcc.9-ensbl1.tex <==
63.14 $\pm$0.00   &  80.17  &  43.45  &  55.56  &  34.54 

==> modell-vqa4-125-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-minAcc.9-ensbl2.tex <==
63.04 $\pm$0.00   &  79.97  &  42.43  &  55.77  &  34.62 

==> modell-vqa4-125-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-minAcc.9-ensbl3.tex <==
63.27 $\pm$0.00   &  80.31  &  42.82  &  55.88  &  34.71 

==> modell-vqa4-135-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-answers6-ensbl1.tex <==
63.32 $\pm$0.00   &  80.22  &  43.05  &  55.99  &  34.39 

==> modell-vqa4-135-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-answers6-ensbl2.tex <==
63.19 $\pm$0.00   &  80.27  &  42.68  &  55.79  &  34.41 

==> modell-vqa4-135-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-answers6-ensbl3.tex <==
63.27 $\pm$0.00   &  80.20  &  43.08  &  55.88  &  34.69 

==> modell-vqa4-140-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-answers10-ensbl1.tex <==
63.37 $\pm$0.00   &  80.49  &  42.93  &  55.91  &  34.64 

==> modell-vqa4-140-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-answers10-ensbl2.tex <==
63.26 $\pm$0.00   &  80.25  &  42.66  &  55.94  &  34.70 

==> modell-vqa4-140-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-answers10-ensbl3.tex <==
63.26 $\pm$0.00   &  80.26  &  43.49  &  55.72  &  34.73 

==> modell-vqa4-140-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-answers12-ensbl1.tex <==
63.22 $\pm$0.00   &  80.40  &  43.19  &  55.61  &  34.69 

==> modell-vqa4-140-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-answers12-ensbl3.tex <==
63.11 $\pm$0.00   &  79.97  &  43.16  &  55.71  &  34.44 

==> modell-vqa4-140-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-answers14-ensbl1.tex <==
63.18 $\pm$0.00   &  80.23  &  43.16  &  55.66  &  34.55 

==> modell-vqa4-140-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-answers14-ensbl2.tex <==
63.31 $\pm$0.00   &  80.52  &  43.13  &  55.71  &  34.98 

==> modell-vqa4-140-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-answers14-ensbl3.tex <==
63.31 $\pm$0.00   &  80.61  &  42.92  &  55.71  &  34.96 

==> modell-vqa4-140-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-answers16-ensbl1.tex <==
63.06 $\pm$0.00   &  80.12  &  42.98  &  55.55  &  34.34 

==> modell-vqa4-140-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-answers16-ensbl2.tex <==
63.19 $\pm$0.00   &  80.23  &  43.11  &  55.69  &  34.60 

==> modell-vqa4-140-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-answers16-ensbl3.tex <==
63.25 $\pm$0.00   &  80.52  &  42.74  &  55.70  &  34.91 

==> modell-vqa4-145-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-answers20-ensbl1.tex <==
63.18 $\pm$0.00   &  80.41  &  42.82  &  55.61  &  34.85 

==> modell-vqa4-145-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-answers20-ensbl2.tex <==
63.08 $\pm$0.00   &  80.04  &  42.99  &  55.65  &  34.55 

==> modell-vqa4-145-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-answers20-ensbl3.tex <==
63.15 $\pm$0.00   &  80.17  &  42.90  &  55.72  &  34.63 

==> modell-vqa4-150-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-answers200-ensbl1.tex <==
59.63 $\pm$0.00   &  79.98  &  42.32  &  48.91  &  32.68 

==> modell-vqa4-150-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-answers200-ensbl2.tex <==
59.57 $\pm$0.00   &  79.91  &  42.04  &  48.90  &  32.71 

==> modell-vqa4-150-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-answers200-ensbl3.tex <==
59.56 $\pm$0.00   &  79.81  &  41.97  &  48.98  &  32.54 

==> modell-vqa4-155-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-qEncG100-ensbl1.tex <==
62.45 $\pm$0.00   &  78.79  &  42.15  &  55.55  &  33.48 

==> modell-vqa4-155-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-qEncG100-ensbl2.tex <==
62.50 $\pm$0.00   &  79.12  &  41.88  &  55.46  &  33.86 

==> modell-vqa4-155-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-qEncG100-ensbl3.tex <==
62.40 $\pm$0.00   &  78.61  &  42.34  &  55.52  &  33.76 

==> modell-vqa4-160-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-qEncG200-ensbl1.tex <==
63.09 $\pm$0.00   &  79.83  &  42.71  &  55.90  &  34.51 

==> modell-vqa4-160-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-qEncG200-ensbl2.tex <==
62.90 $\pm$0.00   &  79.78  &  42.44  &  55.64  &  34.28 

==> modell-vqa4-160-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-qEncG200-ensbl3.tex <==
62.88 $\pm$0.00   &  79.65  &  42.33  &  55.70  &  34.24 

==> modell-vqa4-165-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-qEnc4sumGlove-ensbl1.tex <==
62.11 $\pm$0.00   &  79.67  &  41.82  &  54.29  &  33.82 

==> modell-vqa4-165-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-qEnc4sumGlove-ensbl2.tex <==
62.18 $\pm$0.00   &  79.75  &  41.90  &  54.33  &  34.00 

==> modell-vqa4-165-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-qEnc4sumGlove-ensbl3.tex <==
62.12 $\pm$0.00   &  79.20  &  41.93  &  54.62  &  33.37 

==> modell-vqa4-170-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-qEnc5avgGlove-ensbl1.tex <==
62.62 $\pm$0.00   &  80.22  &  42.33  &  54.76  &  34.34 

==> modell-vqa4-170-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-qEnc5avgGlove-ensbl2.tex <==
62.53 $\pm$0.00   &  80.12  &  42.19  &  54.68  &  34.11 

==> modell-vqa4-170-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-qEnc5avgGlove-ensbl3.tex <==
62.45 $\pm$0.00   &  80.17  &  41.94  &  54.56  &  34.21 

==> modell-vqa4-175-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-qEnc30gruScratch-ensbl1.tex <==
62.21 $\pm$0.00   &  78.85  &  41.65  &  55.14  &  33.67 

==> modell-vqa4-175-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-qEnc30gruScratch-ensbl2.tex <==
62.28 $\pm$0.00   &  78.73  &  41.76  &  55.35  &  33.73 

==> modell-vqa4-175-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-qEnc30gruScratch-ensbl3.tex <==
62.33 $\pm$0.00   &  78.72  &  42.35  &  55.30  &  33.61 

==> modell-vqa4-180-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-qEnc61backward-ensbl1.tex <==
62.85 $\pm$0.00   &  79.55  &  42.54  &  55.67  &  34.07 

==> modell-vqa4-180-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-qEnc61backward-ensbl2.tex <==
62.80 $\pm$0.00   &  79.62  &  42.39  &  55.56  &  33.81 

==> modell-vqa4-180-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-qEnc61backward-ensbl3.tex <==
62.82 $\pm$0.00   &  79.54  &  42.24  &  55.69  &  34.04 

==> modell-vqa4-185-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-qEnc63bidir-ensbl1.tex <==
62.19 $\pm$0.00   &  78.52  &  42.26  &  55.19  &  33.47 

==> modell-vqa4-185-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-qEnc63bidir-ensbl2.tex <==
62.28 $\pm$0.00   &  78.57  &  42.38  &  55.30  &  33.50 

==> modell-vqa4-185-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-qEnc63bidir-ensbl3.tex <==
62.39 $\pm$0.00   &  78.89  &  42.63  &  55.22  &  33.72 

==> modell-vqa4-186-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-qEncRandGlove-ensbl1.tex <==
62.25 $\pm$0.00   &  78.77  &  41.67  &  55.27  &  33.33 

==> modell-vqa4-186-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-qEncRandGlove-ensbl2.tex <==
62.09 $\pm$0.00   &  78.70  &  41.49  &  55.05  &  33.35 

==> modell-vqa4-186-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-qEncRandGlove-ensbl3.tex <==
62.15 $\pm$0.00   &  78.74  &  42.04  &  55.01  &  33.65 

==> modell-vqa4-190-b1s1o8vg1-g300e512-e-1_60_1_1_1_-8-a1-img-ensbl1.tex <==
56.32 $\pm$0.00   &  75.99  &  36.54  &  46.77  &  26.08 

==> modell-vqa4-190-b1s1o8vg1-g300e512-e-1_60_1_1_1_-8-a1-img-ensbl2.tex <==
56.10 $\pm$0.00   &  76.16  &  36.33  &  46.25  &  26.03 

==> modell-vqa4-190-b1s1o8vg1-g300e512-e-1_60_1_1_1_-8-a1-img-ensbl3.tex <==
56.07 $\pm$0.00   &  75.51  &  36.29  &  46.69  &  25.67 

==> modell-vqa4-195-b1s1o8vg1-g300e512-e-1_60_1_20_1_-8-a1-img-ensbl1.tex <==
57.87 $\pm$0.00   &  76.61  &  36.19  &  49.53  &  27.61 

==> modell-vqa4-195-b1s1o8vg1-g300e512-e-1_60_1_20_1_-8-a1-img-ensbl2.tex <==
58.20 $\pm$0.00   &  76.40  &  36.93  &  50.14  &  28.15 

==> modell-vqa4-195-b1s1o8vg1-g300e512-e-1_60_1_20_1_-8-a1-img-ensbl3.tex <==
57.71 $\pm$0.00   &  75.50  &  35.62  &  50.18  &  27.17 

==> modell-vqa4-200-b1s1o8vg1-g300e512-e-1_60_1_30_1_-8-a1-img-ensbl1.tex <==
59.42 $\pm$0.00   &  77.57  &  37.70  &  51.53  &  29.47 

==> modell-vqa4-200-b1s1o8vg1-g300e512-e-1_60_1_30_1_-8-a1-img-ensbl2.tex <==
59.24 $\pm$0.00   &  77.16  &  37.77  &  51.46  &  29.50 

==> modell-vqa4-200-b1s1o8vg1-g300e512-e-1_60_1_30_1_-8-a1-img-ensbl3.tex <==
59.39 $\pm$0.00   &  77.30  &  37.74  &  51.66  &  29.51 

==> modell-vqa4-205-b1s1o8vg1-g300e512-e-1_60_1_40_1_-8-a1-img-ensbl1.tex <==
62.81 $\pm$0.00   &  79.87  &  42.57  &  55.34  &  34.19 

==> modell-vqa4-205-b1s1o8vg1-g300e512-e-1_60_1_40_1_-8-a1-img-ensbl2.tex <==
62.68 $\pm$0.00   &  79.71  &  42.18  &  55.30  &  33.89 

==> modell-vqa4-205-b1s1o8vg1-g300e512-e-1_60_1_40_1_-8-a1-img-ensbl3.tex <==
62.96 $\pm$0.00   &  80.18  &  42.56  &  55.40  &  34.45 

==> modell-vqa4-220-b1s1o8vg1-g300e512-e-1_60_1_30_1_-8-img30att2-ensbl1.tex <==
59.28 $\pm$0.00   &  77.01  &  37.87  &  51.61  &  29.49 

==> modell-vqa4-220-b1s1o8vg1-g300e512-e-1_60_1_30_1_-8-img30att2-ensbl2.tex <==
59.04 $\pm$0.00   &  76.60  &  36.78  &  51.75  &  29.36 

==> modell-vqa4-220-b1s1o8vg1-g300e512-e-1_60_1_30_1_-8-img30att2-ensbl3.tex <==
59.27 $\pm$0.00   &  77.31  &  37.90  &  51.37  &  29.45 

==> modell-vqa4-225-b1s1o8vg1-g300e512-e-1_60_1_30_1_-8-img30att-1-ensbl1.tex <==
58.54 $\pm$0.00   &  76.38  &  37.90  &  50.59  &  27.86 

==> modell-vqa4-225-b1s1o8vg1-g300e512-e-1_60_1_30_1_-8-img30att-1-ensbl2.tex <==
59.14 $\pm$0.00   &  77.35  &  38.00  &  51.05  &  29.03 

==> modell-vqa4-225-b1s1o8vg1-g300e512-e-1_60_1_30_1_-8-img30att-1-ensbl3.tex <==
59.19 $\pm$0.00   &  77.42  &  38.09  &  51.07  &  29.14 

==> modell-vqa4-230-b1s1o8vg1-g300e512-e-1_60_1_30_1_-8-img30att-2-ensbl1.tex <==
59.00 $\pm$0.00   &  77.14  &  38.04  &  50.92  &  29.25 

==> modell-vqa4-230-b1s1o8vg1-g300e512-e-1_60_1_30_1_-8-img30att-2-ensbl2.tex <==
58.69 $\pm$0.00   &  76.74  &  38.04  &  50.59  &  28.64 

==> modell-vqa4-230-b1s1o8vg1-g300e512-e-1_60_1_30_1_-8-img30att-2-ensbl3.tex <==
58.41 $\pm$0.00   &  75.40  &  37.78  &  51.09  &  27.32 

==> modell-vqa4-235-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-img51att2-ensbl1.tex <==
63.07 $\pm$0.00   &  79.86  &  43.14  &  55.72  &  34.64 

==> modell-vqa4-235-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-img51att2-ensbl2.tex <==
63.07 $\pm$0.00   &  79.44  &  43.16  &  56.04  &  34.17 

==> modell-vqa4-235-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-img51att2-ensbl3.tex <==
63.15 $\pm$0.00   &  80.09  &  43.21  &  55.70  &  34.75 

==> modell-vqa4-240-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-img51att-1-ensbl1.tex <==
60.53 $\pm$0.00   &  76.61  &  41.53  &  53.46  &  30.37 

==> modell-vqa4-240-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-img51att-1-ensbl2.tex <==
62.99 $\pm$0.00   &  79.99  &  44.33  &  55.15  &  34.36 

==> modell-vqa4-240-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-img51att-1-ensbl3.tex <==
62.95 $\pm$0.00   &  79.88  &  44.45  &  55.11  &  34.22 

==> modell-vqa4-245-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-img51att-2-ensbl1.tex <==
62.64 $\pm$0.00   &  79.46  &  43.49  &  55.06  &  34.06 

==> modell-vqa4-245-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-img51att-2-ensbl2.tex <==
62.95 $\pm$0.00   &  79.80  &  43.96  &  55.32  &  34.25 

==> modell-vqa4-245-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-img51att-2-ensbl3.tex <==
63.15 $\pm$0.00   &  79.96  &  44.51  &  55.45  &  34.59 

==> modell-vqa4-250-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.1-ensbl1.tex <==
53.42 $\pm$0.00   &  70.52  &  34.43  &  45.58  &  24.50 

==> modell-vqa4-250-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.1-ensbl2.tex <==
53.53 $\pm$0.00   &  69.96  &  35.94  &  45.84  &  24.18 

==> modell-vqa4-250-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.1-ensbl3.tex <==
52.72 $\pm$0.00   &  68.62  &  34.68  &  45.54  &  23.36 

==> modell-vqa4-250-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.1-outRand11-ensbl1.tex <==
51.82 $\pm$0.00   &  69.40  &  33.23  &  43.52  &  23.09 

==> modell-vqa4-250-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.1-outRand11-ensbl2.tex <==
51.17 $\pm$0.00   &  66.99  &  34.68  &  43.65  &  22.06 

==> modell-vqa4-250-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.1-outRand11-ensbl3.tex <==
51.56 $\pm$0.00   &  68.35  &  34.06  &  43.57  &  22.23 

==> modell-vqa4-250-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.1-outRand11.tex <==
51.52 $\pm$0.33   &  68.25  &  33.99  &  43.58  &  22.46 

==> modell-vqa4-250-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.1-qenc30-ensbl1.tex <==
49.88 $\pm$0.00   &  67.38  &  33.65  &  41.01  &  21.34 

==> modell-vqa4-250-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.1-qenc30-ensbl2.tex <==
50.88 $\pm$0.00   &  67.89  &  33.20  &  42.77  &  21.39 

==> modell-vqa4-250-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.1-qenc30-ensbl3.tex <==
46.16 $\pm$0.00   &  66.20  &  28.60  &  35.74  &  18.33 

==> modell-vqa4-250-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.1-qenc30-outRand11-ensbl1.tex <==
49.03 $\pm$0.00   &  66.91  &  30.99  &  40.37  &  20.07 

==> modell-vqa4-250-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.1-qenc30-outRand11-ensbl2.tex <==
48.68 $\pm$0.00   &  67.41  &  33.11  &  38.70  &  20.77 

==> modell-vqa4-250-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.1-qenc30-outRand11-ensbl3.tex <==
49.00 $\pm$0.00   &  65.46  &  32.16  &  41.09  &  20.29 

==> modell-vqa4-250-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.1-qenc30-outRand11.tex <==
48.91 $\pm$0.20   &  66.60  &  32.09  &  40.05  &  20.38 

==> modell-vqa4-250-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.1-qenc30.tex <==
48.98 $\pm$2.49   &  67.16  &  31.82  &  39.84  &  20.35 

==> modell-vqa4-250-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.1.tex <==
53.22 $\pm$0.44   &  69.70  &  35.02  &  45.65  &  24.01 

==> modell-vqa4-255-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.3-ensbl1.tex <==
58.58 $\pm$0.00   &  75.57  &  38.04  &  51.24  &  29.44 

==> modell-vqa4-255-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.3-ensbl2.tex <==
58.36 $\pm$0.00   &  75.08  &  37.98  &  51.19  &  29.04 

==> modell-vqa4-255-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.3-ensbl3.tex <==
58.35 $\pm$0.00   &  75.08  &  38.47  &  51.04  &  29.03 

==> modell-vqa4-255-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.3-outRand11-ensbl1.tex <==
57.56 $\pm$0.00   &  75.00  &  38.63  &  49.47  &  28.71 

==> modell-vqa4-255-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.3-outRand11-ensbl2.tex <==
57.07 $\pm$0.00   &  73.88  &  37.34  &  49.65  &  27.59 

==> modell-vqa4-255-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.3-outRand11-ensbl3.tex <==
57.45 $\pm$0.00   &  75.03  &  37.96  &  49.39  &  28.73 

==> modell-vqa4-255-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.3-outRand11.tex <==
57.36 $\pm$0.26   &  74.64  &  37.98  &  49.50  &  28.34 

==> modell-vqa4-255-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.3-qenc30-ensbl1.tex <==
57.26 $\pm$0.00   &  73.80  &  37.85  &  49.96  &  28.12 

==> modell-vqa4-255-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.3-qenc30-ensbl2.tex <==
56.20 $\pm$0.00   &  72.03  &  37.67  &  49.21  &  26.99 

==> modell-vqa4-255-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.3-qenc30-ensbl3.tex <==
55.82 $\pm$0.00   &  70.88  &  36.55  &  49.60  &  25.76 

==> modell-vqa4-255-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.3-qenc30-outRand11-ensbl1.tex <==
55.64 $\pm$0.00   &  71.70  &  36.62  &  48.61  &  26.37 

==> modell-vqa4-255-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.3-qenc30-outRand11-ensbl2.tex <==
56.15 $\pm$0.00   &  73.18  &  37.06  &  48.40  &  27.10 

==> modell-vqa4-255-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.3-qenc30-outRand11-ensbl3.tex <==
56.31 $\pm$0.00   &  73.39  &  37.53  &  48.44  &  27.47 

==> modell-vqa4-255-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.3-qenc30-outRand11.tex <==
56.04 $\pm$0.35   &  72.75  &  37.07  &  48.48  &  26.98 

==> modell-vqa4-255-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.3-qenc30.tex <==
56.43 $\pm$0.75   &  72.23  &  37.35  &  49.59  &  26.96 

==> modell-vqa4-255-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.3.tex <==
58.43 $\pm$0.13   &  75.24  &  38.16  &  51.16  &  29.17 

==> modell-vqa4-260-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.5-ensbl1.tex <==
60.69 $\pm$0.00   &  77.70  &  40.69  &  53.20  &  31.51 

==> modell-vqa4-260-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.5-ensbl2.tex <==
60.63 $\pm$0.00   &  77.50  &  40.83  &  53.19  &  31.71 

==> modell-vqa4-260-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.5-ensbl3.tex <==
60.58 $\pm$0.00   &  77.38  &  40.65  &  53.23  &  31.37 

==> modell-vqa4-260-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.5-outRand11-ensbl1.tex <==
59.83 $\pm$0.00   &  76.86  &  40.20  &  52.21  &  31.01 

==> modell-vqa4-260-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.5-outRand11-ensbl2.tex <==
59.66 $\pm$0.00   &  76.73  &  39.50  &  52.16  &  30.55 

==> modell-vqa4-260-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.5-outRand11-ensbl3.tex <==
59.72 $\pm$0.00   &  76.84  &  39.96  &  52.09  &  30.91 

==> modell-vqa4-260-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.5-outRand11.tex <==
59.74 $\pm$0.08   &  76.81  &  39.88  &  52.15  &  30.82 

==> modell-vqa4-260-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.5-qenc30-ensbl1.tex <==
59.41 $\pm$0.00   &  75.58  &  40.05  &  52.38  &  30.31 

==> modell-vqa4-260-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.5-qenc30-ensbl2.tex <==
59.49 $\pm$0.00   &  75.48  &  39.44  &  52.78  &  30.01 

==> modell-vqa4-260-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.5-qenc30-ensbl3.tex <==
59.73 $\pm$0.00   &  76.31  &  39.77  &  52.55  &  30.81 

==> modell-vqa4-260-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.5-qenc30-outRand11-ensbl1.tex <==
58.99 $\pm$0.00   &  75.83  &  38.92  &  51.64  &  29.57 

==> modell-vqa4-260-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.5-qenc30-outRand11-ensbl2.tex <==
58.25 $\pm$0.00   &  74.54  &  39.01  &  51.09  &  29.15 

==> modell-vqa4-260-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.5-qenc30-outRand11-ensbl3.tex <==
57.89 $\pm$0.00   &  74.23  &  38.70  &  50.70  &  28.43 

==> modell-vqa4-260-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.5-qenc30-outRand11.tex <==
58.38 $\pm$0.56   &  74.86  &  38.87  &  51.14  &  29.05 

==> modell-vqa4-260-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.5-qenc30.tex <==
59.54 $\pm$0.16   &  75.79  &  39.75  &  52.57  &  30.38 

==> modell-vqa4-260-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.5.tex <==
60.64 $\pm$0.05   &  77.53  &  40.72  &  53.21  &  31.53 

==> modell-vqa4-265-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.7-ensbl1.tex <==
61.81 $\pm$0.00   &  78.73  &  41.10  &  54.57  &  33.01 

==> modell-vqa4-265-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.7-ensbl2.tex <==
62.05 $\pm$0.00   &  79.03  &  41.72  &  54.65  &  33.34 

==> modell-vqa4-265-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.7-ensbl3.tex <==
61.96 $\pm$0.00   &  78.88  &  41.95  &  54.53  &  32.92 

==> modell-vqa4-265-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.7-outRand11-ensbl2.tex <==
60.98 $\pm$0.00   &  78.24  &  40.18  &  53.51  &  32.12 

==> modell-vqa4-265-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.7-outRand11-ensbl3.tex <==
61.14 $\pm$0.00   &  78.41  &  40.92  &  53.52  &  32.51 

==> modell-vqa4-265-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.7-outRand11.tex <==
61.06 $\pm$0.12   &  78.32  &  40.55  &  53.51  &  32.31 

==> modell-vqa4-265-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.7-qenc30-ensbl1.tex <==
60.76 $\pm$0.00   &  77.40  &  41.05  &  53.46  &  31.86 

==> modell-vqa4-265-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.7-qenc30-ensbl2.tex <==
60.38 $\pm$0.00   &  76.79  &  39.77  &  53.51  &  31.45 

==> modell-vqa4-265-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.7-qenc30-ensbl3.tex <==
60.95 $\pm$0.00   &  77.47  &  40.83  &  53.86  &  32.17 

==> modell-vqa4-265-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.7-qenc30-outRand11-ensbl1.tex <==
60.34 $\pm$0.00   &  77.00  &  40.84  &  52.97  &  31.42 

==> modell-vqa4-265-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.7-qenc30-outRand11-ensbl2.tex <==
60.12 $\pm$0.00   &  76.99  &  40.23  &  52.71  &  31.50 

==> modell-vqa4-265-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.7-qenc30-outRand11-ensbl3.tex <==
60.18 $\pm$0.00   &  76.93  &  40.51  &  52.80  &  31.17 

==> modell-vqa4-265-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.7-qenc30-outRand11.tex <==
60.21 $\pm$0.11   &  76.97  &  40.52  &  52.83  &  31.36 

==> modell-vqa4-265-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.7-qenc30.tex <==
60.70 $\pm$0.29   &  77.22  &  40.55  &  53.61  &  31.83 

==> modell-vqa4-265-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.7.tex <==
61.94 $\pm$0.12   &  78.88  &  41.59  &  54.59  &  33.09 

==> modell-vqa4-270-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.9-ensbl1.tex <==
62.78 $\pm$0.00   &  79.74  &  42.18  &  55.49  &  34.04 

==> modell-vqa4-270-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.9-ensbl2.tex <==
62.73 $\pm$0.00   &  79.65  &  42.33  &  55.41  &  34.00 

==> modell-vqa4-270-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.9-ensbl3.tex <==
62.75 $\pm$0.00   &  79.81  &  42.41  &  55.32  &  34.44 

==> modell-vqa4-270-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.9-outRand11-ensbl2.tex <==
62.36 $\pm$0.00   &  79.55  &  41.91  &  54.84  &  33.90 

==> modell-vqa4-270-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.9-outRand11-ensbl3.tex <==
62.36 $\pm$0.00   &  79.53  &  41.97  &  54.85  &  33.57 

==> modell-vqa4-270-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.9-outRand11.tex <==
62.36 $\pm$0.00   &  79.54  &  41.94  &  54.85  &  33.74 

==> modell-vqa4-270-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.9-qenc30-ensbl1.tex <==
61.67 $\pm$0.00   &  77.95  &  41.41  &  54.79  &  32.67 

==> modell-vqa4-270-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.9-qenc30-ensbl2.tex <==
62.00 $\pm$0.00   &  78.76  &  41.63  &  54.78  &  33.41 

==> modell-vqa4-270-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.9-qenc30-ensbl3.tex <==
62.13 $\pm$0.00   &  78.64  &  42.17  &  55.01  &  33.53 

==> modell-vqa4-270-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.9-qenc30-outRand11-ensbl1.tex <==
61.61 $\pm$0.00   &  78.41  &  41.52  &  54.30  &  32.91 

==> modell-vqa4-270-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.9-qenc30-outRand11-ensbl2.tex <==
61.43 $\pm$0.00   &  78.30  &  40.89  &  54.19  &  32.63 

==> modell-vqa4-270-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.9-qenc30-outRand11-ensbl3.tex <==
61.67 $\pm$0.00   &  78.45  &  41.52  &  54.39  &  33.21 

==> modell-vqa4-270-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.9-qenc30-outRand11.tex <==
61.57 $\pm$0.12   &  78.39  &  41.31  &  54.29  &  32.92 

==> modell-vqa4-270-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.9-qenc30.tex <==
61.93 $\pm$0.24   &  78.45  &  41.74  &  54.86  &  33.20 

==> modell-vqa4-270-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset.9.tex <==
62.76 $\pm$0.02   &  79.73  &  42.31  &  55.41  &  34.16 

==> modell-vqa4-270-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset1.0-qenc30-outRand11-ensbl1.tex <==
61.47 $\pm$0.00   &  77.80  &  41.62  &  54.46  &  32.61 

==> modell-vqa4-270-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset1.0-qenc30-outRand11-ensbl2.tex <==
61.89 $\pm$0.00   &  78.73  &  42.17  &  54.45  &  33.21 

==> modell-vqa4-270-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset1.0-qenc30-outRand11-ensbl3.tex <==
61.96 $\pm$0.00   &  78.88  &  41.52  &  54.64  &  33.56 

==> modell-vqa4-270-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-subset1.0-qenc30-outRand11.tex <==
61.77 $\pm$0.26   &  78.47  &  41.77  &  54.52  &  33.12 

==> modell-vqa4-275-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-emb256-ensbl1.tex <==
62.79 $\pm$0.00   &  79.63  &  42.54  &  55.49  &  33.99 

==> modell-vqa4-275-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-emb256-ensbl2.tex <==
62.85 $\pm$0.00   &  79.61  &  42.44  &  55.66  &  34.23 

==> modell-vqa4-275-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-emb256-ensbl3.tex <==
62.74 $\pm$0.00   &  79.62  &  42.39  &  55.45  &  34.13 

==> modell-vqa4-280-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-emb384-ensbl1.tex <==
63.16 $\pm$0.00   &  80.09  &  43.00  &  55.77  &  34.54 

==> modell-vqa4-280-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-emb384-ensbl2.tex <==
63.20 $\pm$0.00   &  80.17  &  43.15  &  55.75  &  34.70 

==> modell-vqa4-280-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-emb384-ensbl3.tex <==
63.00 $\pm$0.00   &  79.92  &  42.51  &  55.71  &  34.40 

==> modell-vqa4-285-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-emb768-ensbl1.tex <==
63.33 $\pm$0.00   &  80.54  &  42.90  &  55.81  &  34.93 

==> modell-vqa4-285-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-emb768-ensbl2.tex <==
63.37 $\pm$0.00   &  80.43  &  43.05  &  55.92  &  34.80 

==> modell-vqa4-285-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-emb768-ensbl3.tex <==
63.44 $\pm$0.00   &  80.54  &  42.58  &  56.10  &  35.09 

==> modell-vqa4-285-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-emb768.tex <==
63.38 $\pm$0.05   &  80.50  &  42.84  &  55.94  &  34.94 

==> modell-vqa4-290-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-emb1024-ensbl1.tex <==
62.40 $\pm$0.00   &  78.65  &  42.64  &  55.41  &  33.43 

==> modell-vqa4-290-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-emb1024-ensbl2.tex <==
63.44 $\pm$0.00   &  80.57  &  42.81  &  56.02  &  34.89 

==> modell-vqa4-290-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-emb1024-ensbl3.tex <==
63.21 $\pm$0.00   &  80.41  &  42.60  &  55.74  &  34.69 

==> modell-vqa4-295-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-emb1280-ensbl1.tex <==
63.36 $\pm$0.00   &  80.51  &  42.74  &  55.92  &  34.87 

==> modell-vqa4-295-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-emb1280-ensbl2.tex <==
63.59 $\pm$0.00   &  80.50  &  43.35  &  56.24  &  35.00 

==> modell-vqa4-295-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-emb1280-ensbl3.tex <==
63.17 $\pm$0.00   &  80.19  &  42.97  &  55.72  &  34.41 

==> modell-vqa4-300-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-blockRelu-ensbl1.tex <==
61.84 $\pm$0.00   &  78.78  &  41.26  &  54.56  &  33.03 

==> modell-vqa4-300-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-blockRelu-ensbl2.tex <==
61.42 $\pm$0.00   &  78.24  &  40.98  &  54.19  &  32.08 

==> modell-vqa4-300-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-blockRelu-ensbl3.tex <==
61.64 $\pm$0.00   &  78.43  &  41.20  &  54.43  &  32.59 

==> modell-vqa4-305-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-blockTanh-ensbl1.tex <==
62.12 $\pm$0.00   &  79.82  &  40.45  &  54.55  &  33.66 

==> modell-vqa4-305-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-blockTanh-ensbl2.tex <==
61.26 $\pm$0.00   &  78.69  &  41.20  &  53.47  &  32.61 

==> modell-vqa4-305-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-blockTanh-ensbl3.tex <==
61.85 $\pm$0.00   &  79.08  &  41.12  &  54.38  &  33.03 

==> modell-vqa4-310-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-blockGatedRelu-ensbl1.tex <==
62.51 $\pm$0.00   &  79.35  &  42.33  &  55.20  &  33.71 

==> modell-vqa4-310-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-blockGatedRelu-ensbl2.tex <==
62.44 $\pm$0.00   &  79.27  &  42.12  &  55.17  &  33.51 

==> modell-vqa4-310-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-blockGatedRelu-ensbl3.tex <==
62.38 $\pm$0.00   &  79.37  &  41.91  &  55.02  &  33.33 

==> modell-vqa4-315-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-batch128-ensbl1.tex <==
62.32 $\pm$0.00   &  79.75  &  42.10  &  54.57  &  34.01 

==> modell-vqa4-315-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-batch128-ensbl3.tex <==
62.44 $\pm$0.00   &  79.66  &  42.47  &  54.78  &  34.01 

==> modell-vqa4-320-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-batch256-ensbl1.tex <==
63.15 $\pm$0.00   &  80.34  &  43.08  &  55.54  &  34.67 

==> modell-vqa4-320-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-batch256-ensbl2.tex <==
63.27 $\pm$0.00   &  80.20  &  43.14  &  55.87  &  34.57 

==> modell-vqa4-320-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-batch256-ensbl3.tex <==
63.10 $\pm$0.00   &  80.11  &  42.60  &  55.74  &  34.90 

==> modell-vqa4-325-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-batch384-ensbl1.tex <==
63.16 $\pm$0.00   &  80.22  &  42.94  &  55.68  &  34.72 

==> modell-vqa4-325-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-batch384-ensbl2.tex <==
63.22 $\pm$0.00   &  80.26  &  43.07  &  55.75  &  34.58 

==> modell-vqa4-325-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-batch384-ensbl3.tex <==
63.23 $\pm$0.00   &  80.14  &  43.21  &  55.82  &  34.54 

==> modell-vqa4-330-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-batch768-ensbl1.tex <==
63.08 $\pm$0.00   &  80.16  &  42.82  &  55.60  &  34.74 

==> modell-vqa4-330-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-batch768-ensbl2.tex <==
63.05 $\pm$0.00   &  79.98  &  42.46  &  55.77  &  34.36 

==> modell-vqa4-330-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-a1-batch768-ensbl3.tex <==
62.85 $\pm$0.00   &  79.37  &  42.54  &  55.82  &  34.09 

==> modell-vqa4-335-b1s1o8vg1-g300e512-e-1_60_1_51_1_-5-out-ensbl1.tex <==
62.45 $\pm$0.00   &  79.88  &  40.80  &  55.07  &  33.73 

==> modell-vqa4-335-b1s1o8vg1-g300e512-e-1_60_1_51_1_-5-out-ensbl2.tex <==
62.65 $\pm$0.00   &  80.28  &  41.06  &  55.12  &  34.25 

==> modell-vqa4-335-b1s1o8vg1-g300e512-e-1_60_1_51_1_-5-out-ensbl3.tex <==
62.53 $\pm$0.00   &  79.99  &  41.03  &  55.09  &  33.98 

==> modell-vqa4-335-b1s1o8vg1-g300e512-e-1_60_1_51_1_-5-out.tex <==
62.54 $\pm$0.11   &  80.05  &  40.96  &  55.09  &  33.99 

==> modell-vqa4-340-b1s1o8vg1-g300e512-e-1_60_1_51_1_-7-out-ensbl1.tex <==
62.94 $\pm$0.00   &  79.81  &  43.00  &  55.53  &  34.48 

==> modell-vqa4-340-b1s1o8vg1-g300e512-e-1_60_1_51_1_-7-out-ensbl2.tex <==
62.86 $\pm$0.00   &  80.09  &  42.35  &  55.34  &  34.18 

==> modell-vqa4-340-b1s1o8vg1-g300e512-e-1_60_1_51_1_-7-out-ensbl3.tex <==
62.80 $\pm$0.00   &  79.80  &  42.60  &  55.36  &  34.15 

==> modell-vqa4-340-b1s1o8vg1-g300e512-e-1_60_1_51_1_-7-out.tex <==
62.86 $\pm$0.07   &  79.90  &  42.65  &  55.41  &  34.27 

==> modell-vqa4-345-b1s1o8vg1-g300e512-e-1_60_1_51_1_5-out-ensbl1.tex <==
60.26 $\pm$0.00   &  78.21  &  40.41  &  52.02  &  32.11 

==> modell-vqa4-345-b1s1o8vg1-g300e512-e-1_60_1_51_1_5-out-ensbl2.tex <==
60.20 $\pm$0.00   &  77.96  &  40.27  &  52.13  &  31.94 

==> modell-vqa4-345-b1s1o8vg1-g300e512-e-1_60_1_51_1_5-out-ensbl3.tex <==
60.20 $\pm$0.00   &  78.29  &  40.77  &  51.74  &  32.18 

==> modell-vqa4-345-b1s1o8vg1-g300e512-e-1_60_1_51_1_5-out.tex <==
60.22 $\pm$0.03   &  78.15  &  40.49  &  51.96  &  32.07 

==> modell-vqa4-350-b1s1o8vg1-g300e512-e-1_60_1_51_1_7-out-ensbl1.tex <==
60.21 $\pm$0.00   &  78.08  &  40.97  &  51.88  &  32.14 

==> modell-vqa4-350-b1s1o8vg1-g300e512-e-1_60_1_51_1_7-out-ensbl2.tex <==
60.26 $\pm$0.00   &  78.08  &  41.19  &  51.91  &  32.35 

==> modell-vqa4-350-b1s1o8vg1-g300e512-e-1_60_1_51_1_7-out-ensbl3.tex <==
60.23 $\pm$0.00   &  78.19  &  40.44  &  51.97  &  32.28 

==> modell-vqa4-350-b1s1o8vg1-g300e512-e-1_60_1_51_1_7-out.tex <==
60.24 $\pm$0.02   &  78.11  &  40.87  &  51.92  &  32.26 

==> modell-vqa4-355-b1s1o8vg1-g300e512-e-1_60_1_51_1_8-out-ensbl1.tex <==
60.51 $\pm$0.00   &  77.89  &  40.99  &  52.60  &  31.87 

==> modell-vqa4-355-b1s1o8vg1-g300e512-e-1_60_1_51_1_8-out-ensbl2.tex <==
60.38 $\pm$0.00   &  78.13  &  40.98  &  52.18  &  32.35 

==> modell-vqa4-355-b1s1o8vg1-g300e512-e-1_60_1_51_1_8-out-ensbl3.tex <==
60.52 $\pm$0.00   &  78.54  &  40.80  &  52.19  &  32.61 

==> modell-vqa4-360-b1s1o8vg1-g300e512-e-1_60_1_51_1_-10-outRand-ensbl1.tex <==
63.21 $\pm$0.00   &  80.15  &  42.76  &  55.88  &  34.85 

==> modell-vqa4-360-b1s1o8vg1-g300e512-e-1_60_1_51_1_-10-outRand-ensbl2.tex <==
63.22 $\pm$0.00   &  80.12  &  43.10  &  55.85  &  34.52 

==> modell-vqa4-360-b1s1o8vg1-g300e512-e-1_60_1_51_1_-10-outRand-ensbl3.tex <==
63.20 $\pm$0.00   &  79.91  &  43.05  &  55.97  &  34.59 

==> modell-vqa4-360-b1s1o8vg1-g300e512-e-1_60_1_51_1_-11-outRand-ensbl1.tex <==
62.83 $\pm$0.00   &  79.97  &  42.47  &  55.34  &  34.15 

==> modell-vqa4-360-b1s1o8vg1-g300e512-e-1_60_1_51_1_-11-outRand-ensbl2.tex <==
63.09 $\pm$0.00   &  79.99  &  42.92  &  55.72  &  34.33 

==> modell-vqa4-360-b1s1o8vg1-g300e512-e-1_60_1_51_1_-11-outRand-ensbl3.tex <==
62.89 $\pm$0.00   &  80.01  &  42.78  &  55.35  &  34.30 

==> modell-vqa4-360-b1s1o8vg1-g300e512-e-1_60_1_51_1_-12-outRand-ensbl1.tex <==
62.76 $\pm$0.00   &  79.71  &  42.45  &  55.39  &  33.94 

==> modell-vqa4-360-b1s1o8vg1-g300e512-e-1_60_1_51_1_-12-outRand-ensbl2.tex <==
62.93 $\pm$0.00   &  79.58  &  43.17  &  55.65  &  34.05 

==> modell-vqa4-360-b1s1o8vg1-g300e512-e-1_60_1_51_1_-12-outRand-ensbl3.tex <==
61.14 $\pm$0.00   &  76.22  &  41.88  &  54.91  &  31.44 

==> modell-vqa4-360-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-outRand10-ensbl1.tex <==
62.93 $\pm$0.00   &  79.84  &  42.39  &  55.65  &  34.33 

==> modell-vqa4-360-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-outRand10-ensbl3.tex <==
63.01 $\pm$0.00   &  79.82  &  42.84  &  55.72  &  34.30 

==> modell-vqa4-365-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-outRand01-ensbl1.tex <==
63.05 $\pm$0.00   &  80.45  &  42.44  &  55.42  &  34.78 

==> modell-vqa4-365-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-outRand01-ensbl2.tex <==
63.06 $\pm$0.00   &  80.11  &  43.02  &  55.55  &  34.59 

==> modell-vqa4-365-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-outRand01-ensbl3.tex <==
63.02 $\pm$0.00   &  80.04  &  43.04  &  55.52  &  34.61 

==> modell-vqa4-370-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-outRand11-ensbl1.tex <==
62.80 $\pm$0.00   &  80.06  &  42.47  &  55.21  &  34.23 

==> modell-vqa4-370-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-outRand11-ensbl2.tex <==
62.61 $\pm$0.00   &  79.68  &  42.23  &  55.17  &  34.09 

==> modell-vqa4-370-b1s1o8vg1-g300e512-e-1_60_1_51_1_-8-outRand11-ensbl3.tex <==
62.52 $\pm$0.00   &  79.71  &  42.07  &  55.01  &  34.19 

==> modell-vqaCumul-02-outRand01-addOutText-ensbl1.tex <==
62.89 $\pm$0.00   &  80.12  &  42.46  &  55.35  &  34.28 

==> modell-vqaCumul-02-outRand01-addOutText-ensbl2.tex <==
63.00 $\pm$0.00   &  80.05  &  42.62  &  55.58  &  34.46 

==> modell-vqaCumul-02-outRand01-addOutText-ensbl3.tex <==
63.14 $\pm$0.00   &  80.15  &  43.32  &  55.60  &  34.46 

==> modell-vqaCumul-03-outRand11-addMsrFeatures-ensbl1.tex <==
62.64 $\pm$0.00   &  79.89  &  42.10  &  55.10  &  34.16 

==> modell-vqaCumul-03-outRand11-addMsrFeatures-ensbl2.tex <==
62.75 $\pm$0.00   &  79.81  &  42.95  &  55.17  &  34.35 

==> modell-vqaCumul-03-outRand11-addMsrFeatures-ensbl3.tex <==
62.63 $\pm$0.00   &  79.54  &  42.88  &  55.15  &  34.17 

==> modell-vqaCumul-05-img30-addVg-ensbl1.tex <==
58.80 $\pm$0.00   &  77.00  &  37.44  &  50.78  &  29.15 

==> modell-vqaCumul-05-img30-addVg-ensbl2.tex <==
59.00 $\pm$0.00   &  77.22  &  37.55  &  50.98  &  29.52 

==> modell-vqaCumul-05-img30-addVg-ensbl3.tex <==
58.90 $\pm$0.00   &  77.27  &  36.55  &  51.01  &  29.50 

==> modell-vqaCumul-05-noVg-addShufflePairs-ensbl1.tex <==
57.84 $\pm$0.00   &  77.65  &  36.59  &  48.57  &  28.83 

==> modell-vqaCumul-05-noVg-addShufflePairs-ensbl2.tex <==
57.80 $\pm$0.00   &  77.44  &  36.45  &  48.68  &  28.63 

==> modell-vqaCumul-05-noVg-addShufflePairs-ensbl3.tex <==
57.89 $\pm$0.00   &  77.28  &  37.15  &  48.80  &  28.50 

==> modell-vqaCumul-05-shuffle0-addGlove-ensbl1.tex <==
57.55 $\pm$0.00   &  77.23  &  35.97  &  48.47  &  28.55 

==> modell-vqaCumul-05-shuffle0-addGlove-ensbl2.tex <==
57.66 $\pm$0.00   &  77.24  &  36.72  &  48.49  &  28.51 

==> modell-vqaCumul-05-shuffle0-addGlove-ensbl3.tex <==
57.83 $\pm$0.00   &  77.28  &  36.70  &  48.80  &  28.54 

==> modell-vqaCumul-07-qenc30-replaceTanhByGatedTanh-ensbl1.tex <==
57.21 $\pm$0.00   &  76.28  &  36.11  &  48.46  &  27.78 

==> modell-vqaCumul-07-qenc30-replaceTanhByGatedTanh-ensbl2.tex <==
56.86 $\pm$0.00   &  75.78  &  36.19  &  48.11  &  27.37 

==> modell-vqaCumul-07-qenc30-replaceTanhByGatedTanh-ensbl3.tex <==
56.82 $\pm$0.00   &  75.69  &  35.80  &  48.20  &  27.36 

==> modell-vqaCumul-08-tanh-replaceReluByTanh-ensbl1.tex <==
43.67 $\pm$0.00   &  75.32  &  34.95  &  22.15  &  20.24 

==> modell-vqaCumul-08-tanh-replaceReluByTanh-ensbl2.tex <==
56.34 $\pm$0.00   &  76.09  &  34.26  &  47.34  &  26.84 

==> modell-vqaCumul-08-tanh-replaceReluByTanh-ensbl3.tex <==
56.39 $\pm$0.00   &  76.29  &  34.32  &  47.27  &  27.25 

==> modell-vqaCumul-09-relu-softTargets-ensbl1.tex <==
55.36 $\pm$0.00   &  74.97  &  34.34  &  46.18  &  25.47 

==> modell-vqaCumul-09-relu-softTargets-ensbl2.tex <==
55.44 $\pm$0.00   &  74.81  &  34.57  &  46.41  &  25.42 

==> modell-vqaCumul-09-relu-softTargets-ensbl3.tex <==
55.34 $\pm$0.00   &  74.18  &  35.58  &  46.41  &  24.82 

==> modell-vqaCumul-10-hardTargets-addSigmoidOut-ensbl1.tex <==
55.68 $\pm$0.00   &  75.10  &  35.13  &  46.52  &  25.59 

==> modell-vqaCumul-10-hardTargets-addSigmoidOut-ensbl2.tex <==
56.38 $\pm$0.00   &  75.88  &  34.93  &  47.40  &  26.93 

==> modell-vqaCumul-10-hardTargets-addSigmoidOut-ensbl3.tex <==
55.69 $\pm$0.00   &  74.85  &  36.04  &  46.48  &  25.48 

==> modell-vqaCumul-10-hardTargets-addSigmoidOut.tex <==
55.92 $\pm$0.40   &  75.28  &  35.37  &  46.80  &  26.00 

==> modell-vqaCumul-10-hardTargets.1-ensbl1.tex <==
54.34 $\pm$0.00   &  73.84  &  34.55  &  44.92  &  23.71 

==> modell-vqaCumul-10-hardTargets.1-ensbl2.tex <==
54.15 $\pm$0.00   &  73.78  &  34.69  &  44.53  &  23.65 

==> modell-vqaCumul-10-hardTargets.1-ensbl3.tex <==
54.53 $\pm$0.00   &  73.79  &  34.26  &  45.40  &  23.90 

==> modell-vqaCumul-10-hardTargets.9-ensbl1.tex <==
53.65 $\pm$0.00   &  73.28  &  34.91  &  43.84  &  24.35 

==> modell-vqaCumul-10-hardTargets.9-ensbl2.tex <==
53.33 $\pm$0.00   &  73.18  &  34.22  &  43.45  &  24.42 

==> modell-vqaCumul-10-hardTargets.9-ensbl3.tex <==
53.27 $\pm$0.00   &  73.24  &  34.02  &  43.34  &  24.19 

==> modell-vqaCumul-10b-softmaxOut-worst-ensbl1.tex <==
52.20 $\pm$0.00   &  72.21  &  34.44  &  41.84  &  22.97 

==> modell-vqaCumul-10b-softmaxOut-worst-ensbl2.tex <==
52.80 $\pm$0.00   &  73.30  &  34.02  &  42.35  &  24.15 

==> modell-vqaCumul-10b-softmaxOut-worst-ensbl3.tex <==
52.57 $\pm$0.00   &  72.86  &  34.53  &  42.08  &  24.32 

==> modell-vqaCumul-11-softmaxOut-worst-ensbl1.tex <==
53.09 $\pm$0.00   &  72.87  &  33.52  &  43.40  &  23.95 

==> modell-vqaCumul-11-softmaxOut-worst-ensbl3.tex <==
53.01 $\pm$0.00   &  72.36  &  34.55  &  43.33  &  23.71 

==> modell-vqaCumul-11-softmaxOut-worst.tex <==
53.05 $\pm$0.06   &  72.62  &  34.03  &  43.37  &  23.83 
